Decoupling Task-Solving and Output Formatting in LLM Generation

Large language models (LLMs) are increasingly adept at solving complex problems, such as mathematical reasoning and automatic evaluation. However, performance often degrades when prompts intertwine task instructions with rigid formatting requirements. This entanglement creates competing goals for the model, hindering its reasoning capabilities. To address this, we introduce Deco-G, a decoding framework that explicitly decouples format adherence from problem solving. Deco-G delegates format adherence to a separate Format Estimation Module (FEM), which performs probabilistic lookahead to estimate future format compliance rate and reweighs token probabilities, allowing the LLM to focus solely on task resolution. To make this approach both practical and efficient, we introduce three key innovations: instruction-aware distillation, a flexible trie-building algorithm, and HMM state pruning. Experiments across mathematical reasoning, event argument extraction, and LLM-as-a-judge demonstrate that Deco-G constantly gains over prompting or structured generation baselines, with guaranteed format compliance. We release our code at https://github.com/haikangdeng/deco-g.

==> tables/gsm8k_ace05.tex <==
% Add these packages to your document preamble if you don't have them already
% \usepackage{booktabs}
% \usepackage{caption}
% \usepackage[table]{xcolor}

\definecolor{modelrowcolor}{gray}{0.90}

\begin{table*}[t]
\centering
\footnotesize % Use a smaller font for the entire table environment

% --- First Table (GSM8k Results) ---
\begin{minipage}[t]{0.48\textwidth}
    % \vspace{-.5em}
    % \caption{GSM8k Results. DECO-G guarantees format satisfaction and achieves 85.2\% accuracy with \textit{Llama}, outperforming NL and JSON generations by more than 4.5\% (absolute). With \textit{Qwen}, DECO-G improves accuracy by 3.8\% (absolute).}
    \centering
    \begin{tabular}{l c c}
    \toprule
    \textbf{Method} & \textbf{Format (\%)} & \textbf{Acc. (\%)} \\ % Abbreviated "Compliance" for space
    \midrule
    % Llama-3.1-8B-Instruct
    \rowcolor{modelrowcolor}
    \multicolumn{3}{c}{\textit{Llama-3.1-8B-Instruct}} \\
    \cmidrule(lr){1-3}
    NL & 96.3 & 82.3 \\
    NL-S & 100 & 81.3 \\
    JSON & 64.7 & 51.8\\
    JSON-S & 100 & 75.7 \\
    \textbf{DECO-G} & 100 & \textbf{85.2} \\
    \midrule
    % Qwen-2.5-7B-Instruct
    \rowcolor{modelrowcolor}
    \multicolumn{3}{c}{\textit{Qwen2.5-7B-Instruct}} \\
    \cmidrule(lr){1-3}
    NL & 98.0 & 83.6 \\
    NL-S & 99.9 & 82.7 \\
    JSON & 93.3 & 74.8 \\
    JSON-S & 99.8 & 79.0 \\
    \textbf{DECO-G}$^{\gamma=2}$ & 100 & \textbf{88.6} \\
    \midrule
    \rowcolor{modelrowcolor}
    \multicolumn{3}{c}{\textit{Qwen3-8B}} \\
    \cmidrule(lr){1-3}
    NL & 97.4 & 90.5 \\
    NL-S & 100 & 88.3 \\
    JSON & 66.9 & 61.4 \\
    JSON-S & 99.2 & 90.6 \\
    \textbf{DECO-G}$^{\gamma=2}$ & 100 & \textbf{91.7} \\
    \bottomrule
    \end{tabular}
    % \vspace{-1em}
    \label{tab:gsm8k}
    \caption{GSM8k results.}
\end{minipage}
\hfill % This creates a flexible space between the two minipages
% --- Second Table (EAE Results) ---
\begin{minipage}[t]{0.48\textwidth}
    % \vspace{-.5em}
    % \caption{Generative EAE results on ACE05. \framework improves overall extraction performance for \textit{Llama} and \textit{Qwen}.}
    \centering
    \begin{tabular}{l cccc}
    \toprule
    \textbf{Method} & \textbf{AI} & \textbf{AC} & \textbf{AI+} & \textbf{AC+} \\
    \midrule
    % Llama-3.1-8B-Instruct
    \rowcolor{modelrowcolor}
    \multicolumn{5}{c}{\textit{Llama-3.1-8B-Instruct}} \\
    \cmidrule(lr){1-5}
    NL & 36.8 & 27.3 & 34.8 & 25.5 \\
    NL-S & 37.1 & 27.8 & 35.1 & 26.0 \\
    JSON & 35.2 & 26.2 & 33.4 & 24.6 \\
    JSON-S & 33.6 & 25.2 & 31.6 & 23.6 \\
    \textbf{DECO-G} & \textbf{39.4} & \textbf{28.7} & \textbf{37.0} & \textbf{26.8} \\
    \midrule
    % Qwen-2.5-7B-Instruct
    \rowcolor{modelrowcolor}
    \multicolumn{5}{c}{\textit{Qwen2.5-7B-Instruct}} \\
    \cmidrule(lr){1-5}
    NL & 32.6 & 25.5 & 31.2 & 24.4 \\
    NL-S & 33.2 & 24.9 & 31.1 & 23.7 \\
    JSON & 31.9 & 24.1 & 30.5 & 22.9 \\
    JSON-S & 34.1 & \textbf{26.1} & 32.5 & \textbf{24.7} \\
    \textbf{DECO-G}$^{\gamma=2}$ & \textbf{35.2} & 25.9 & \textbf{33.4} & 24.5 \\
    % DECO-G ($\gamma=3$) & 32.5 & 23.1 & 30.7 & 21.9 \\
    \midrule
    \rowcolor{modelrowcolor}
    \multicolumn{5}{c}{\textit{Qwen3-8B}} \\
    \cmidrule(lr){1-5}
    NL & 33.2 & \textbf{24.6} & 31.5 & \textbf{23.1} \\
    NL-S & 33.3 & 24.2 & 31.5 & 22.6 \\
    JSON & 31.7 & 23.4 & 3.01 & 21.8 \\
    JSON-S & 32.5 & 23.0 & 30.8 & 21.5 \\
    \textbf{DECO-G}$^{\gamma=2}$ & \textbf{34.0} & \textbf{24.6} & \textbf{32.1} & \textbf{23.1} \\
    \bottomrule
    \end{tabular}
    % \vspace{-.5em}
    \label{tab:ace05}
    \caption{Generative EAE results on ACE05.}
\end{minipage}
\end{table*}
